A review of advances in pixel detectors for experiments with high rate and radiation

The Large Hadron Collider (LHC) experiments ATLAS and CMS have established hybrid pixel detectors as the instrument of choice for particle tracking and vertexing in high rate and radiation environments, as they operate close to the LHC interaction points. With the High Luminosity-LHC upgrade now in sight, for which the tracking detectors will be completely replaced, new generations of pixel detectors are being devised. They have to address enormous challenges in terms of data throughput and radiation levels, ionizing and non-ionizing, that harm the sensing and readout parts of pixel detectors alike. Advances in microelectronics and microprocessing technologies now enable large scale detector designs with unprecedented performance in measurement precision (space and time), radiation hard sensors and readout chips, hybridization techniques, lightweight supports, and fully monolithic approaches to meet these challenges. This paper reviews the world-wide effort on these developments.

==> moduleconcepts.tex <==
% ========================================
% ========================================
\section{Module Concepts}\label{sec:modules}
% ========================================
% ========================================

Module concepts:     	postprocessing, bonding, TSVs, wafer to wafer dreams

%
\begin{figure}
\centering
    \includegraphics[width=0.9\textwidth]{figs/test_figure}
\caption{Test figure.}
\label{fig:spezifischerWiderstand}
\end{figure}
%
